Entity Linking via Dual and Cross-Attention Encoders

Entity Linking has two main open areas of research: 1) generate candidate entities without using alias tables and 2) generate more contextual representations for both mentions and entities. Recently, a solution has been proposed for the former as a dual-encoder entity retrieval system (Gillick et al., 2019) that learns mention and entity representations in the same space, and performs linking by selecting the nearest entity to the mention in this space. In this work, we use this retrieval system solely for generating candidate entities. We then rerank the entities by using a cross-attention encoder over the target mention and each of the candidate entities. Whereas a dual encoder approach forces all information to be contained in the small, fixed set of vector dimensions used to represent mentions and entities, a crossattention model allows for the use of detailed information (read: features) from the entirety of each <mention, context, candidate entity> tuple. We experiment with features used in the reranker including different ways of incorporating document-level context. We achieve state-of-the-art results on TACKBP-2010 dataset, with 92.05% accuracy. Furthermore, we show how the rescoring model generalizes well when trained on the larger CoNLL-2003 dataset and evaluated on TACKBP-2010.

==> Entity linking via dual and cross-attention encoders/ablation.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabularx}{\linewidth}{L{0.49}|C{0.1}|C{0.1}|C{0.13}|C{0.12}|C{0.1}|C{0.1}|C{0.3}|C{0.2}}
{\bf Model}   & $m_s$      & $c_l$      & $c_{dm}$     & $c_{db}$     & $e_n$      & $e_d$      & {\bf CoNLL} & {\bf TAC} \\ \hline
DEER R@1      & \multicolumn{6}{c|}{}                                                       & 75.71 & 86.86     \\ \hline
Reranking     & \checkmark &            &            &            & \checkmark &            & 80.69 & 81.76     \\ \hline
Reranking     & \checkmark & \checkmark &            &            & \checkmark &            & 83.34 & 86.27     \\ \hline
Reranking     & \checkmark & \checkmark &            &            & \checkmark & \checkmark & 84.57 & 88.92     \\ \hline
Reranking     & \checkmark & \checkmark & \checkmark &            & \checkmark & \checkmark & 87.12 & -         \\ \hline
Reranking     & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 88.31 & 89.59     \\ 
\end{tabularx} 
\caption{Ablation study for input used in the reranker. Reranker is trained on the CoNLL-2003 training split and evaluated on test splits from both CoNLL-2003 and TACKBP-2010. $m_s$ is the mention span, $c_l$ is the local context (sentence), $c_{dm}$ is the document context (other mentions in the document), $c_{db}$ is the document context (document bag of words), $e_n$ is the entity name and $e_d$ is the entity description. $e_n$ usually appears in $e_d$ and isn't included explicitly when $e_d$ is used. Similarly,  $c_{dm}$ is implicitly included in  $c_{db}$.}
\label{table:Ablation}
\end{table}

==> Entity linking via dual and cross-attention encoders/dataset_stats.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabularx}{\linewidth}{L{0.6}|R{0.35}|R{0.35}|R{0.25}}
{\bf Dataset} & \multicolumn{1}{c|}{\bf Docs} & \multicolumn{1}{c|}{\bf Mentions} & \multicolumn{1}{c}{\bf M/D} \\\hline
CoNLL-03 train & 946 & 18541 & 19.60 \\
CoNLL-03 test & 231 & 4485 & 19.43 \\
TAC-10 train & 1043 & 1059 & 1.01 \\
TAC-10 test & 1013 & 1020 & 1.01 \\
\end{tabularx} 
\caption{Number of documents and mentions in each of the datasets. M/D is the average number of mentions per document.}
\label{table:DatasetStats}
\end{table}


==> Entity linking via dual and cross-attention encoders/fair_comparison.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabularx}{\linewidth}{L{0.65}|C{0.35}}
{\bf Model} & {\bf Accuracy (\%)} \\\hline
\cite{sun2015modeling} & 83.90 \\ %818k entities
\cite{raiman2018deeptype} & 90.85 \\  %1M entities
\cite{gillick-etal-2019-learning} & 88.62 \\
This work & 92.05 \\ \hline
\cite{yamada-etal-2017-learning} & 85.20 \\
\cite{nie2018mention} & 89.10 \\ 
\cite{gillick-etal-2019-learning} & 86.86 \\
This work & 88.42 \\
\end{tabularx} 
\caption{Mention-level accuracy on the TACKBP-2010 test set. Wikipedia is growing immensely with time and the difficulty of the task depends on the number of entities in the knowledge base. The first set of rows use 800k-1M entities and the second set of rows use 5-5.7M entities. This allows for a relatively fair comparison, if not perfectly fair as the number of entities is still not exactly the same.}
\label{table:ComparisonFair}
\end{table}

==> Entity linking via dual and cross-attention encoders/full_comparison.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabularx}{\linewidth}{L{0.6}|C{0.25}|C{0.25}|C{0.26}}
{\bf Model} & {\bf CoNLL} & {\bf TAC} & {\bf TAC transfer} \\\hline
DEER Recall@1 & 75.71 & 86.86 & 86.86\\
DEER Recall@100 & 94.04 & 96.27 & 96.27\\
This work & 88.31 & 88.42 & 89.59 \\
\end{tabularx} 
\caption{Mention-level accuracy (\%) on the TACKBP-2010 and CoNLL-2003 test sets. Knowledge base includes 5.7M entities. Reranker is trained on corresponding training splits of the two datasets for the first two columns. The third column is trained on CoNLL and evaluated on TAC.}
\label{table:ComparisonFull}
\end{table}


==> Entity linking via dual and cross-attention encoders/pred_examples.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{2pt}
\begin{tabularx}{\linewidth}{L{0.12}|L{0.12}|L{0.45}|L{0.35}|L{0.35}}
{\bf Model 1 features} & {\bf Model 2 features} & \multicolumn{1}{c|}{\bf Mention in Context} & \multicolumn{1}{c|}{\bf Model 1 entity} & \multicolumn{1}{c}{\bf Model 2 entity} \\\hline

Top candidate & $m_s$ + $e_n$ & $c_l$ not used - Only for illustration. {\color{red}CZECH} VICE-PM SEES WIDER DEBATE AT PARTY CONGRESS.  & Czech language & Czech Republic \\\hline

$m_s$ + $e_n$  & $m_s$ + $c_l$ + $e_n$ & SOCCER - {\color{red}JAPAN} GET LUCKY WIN, CHINA IN SURPRISE DEFEAT & Japan & Japan national football team \\\hline

$m_s$ + $c_l$ + $e_n$  & $m_s$ + $c_l$ + $e_d$ & CRICKET - {\color{red}LARA} ENDURES ANOTHER MISERABLE DAY & {\em (Lara Dutta)} Lara Dutta is an Indian actress, model and beauty queen who was crowned Miss Intercontinental 1997 and Miss Universe 2000. & {\em (Brian Lara)} Brian Charles Lara is a Trinidadian former international cricketer,[1][2] widely acknowledged as one of the greatest batsmen of all time.) \\\hline

$m_s$ + $c_l$ + $e_d$  & $m_s$ + $c_l$ + $c_d$ + $e_d$ & Police spokeswoman Deborah Denis said Thursday that George Sherryl Whittaker was attacked by scores of honeybees in his yard in the wealthy British dependency's capital, {\color{red}George Town}. & {\em (George Town, Penang)} George Town, the capital city of the Malaysian state of Penang, is located at the north-eastern tip of Penang Island. & {\em (George Town, Cayman Islands)} George Town is a city situated on Grand Cayman island of the Cayman Islands.)  \\
 & & $c_d$: 2008 23:06:18 agitated Cayman swarm year man Wednesday Islands pronounced Firefighters water 74 UTC old bees died attack hoses dead hospital chase attacked 11 shortly 09 & & \\
 
\end{tabularx} 
\caption{Qualitative analysis of reranker with different input features. Reranker is trained on the CoNLL-2003 training split and evaluated on test splits from both CoNLL-2003 and TACKBP-2010. Mention is marked in red in the local context. In each example, model 1 is incorrect and model 2 is correct, illustrating the improvement. $m_s$ is the mention span, $c_l$ is the local context (sentence), $c_d$ is the document context (document bag of words), $e_n$ is the entity name and $e_d$ is the entity description. $e_n$ usually appears in $e_d$ and isn't included explicitly when $e_d$ is used.}
\label{table:Analysis}
\end{table*}

